Entropy-Based Modeling for Estimating Soft Errors Impact on Binarized Neural Network Inference

Over past years, the easy accessibility to the large scale datasets has significantly shifted the paradigm for developing highly accurate prediction models that are driven from Neural Network (NN). These models can be potentially impacted by the radiation-induced transient faults that might lead to the gradual downgrade of the long-running expected NN inference accelerator. The crucial observation from our rigorous vulnerability assessment on the NN inference accelerator demonstrates that the weights and activation functions are unevenly susceptible to both single-event upset (SEU) and multi-bit upset (MBU), especially in the first five layers of our selected convolution neural network. In this paper, we present the relatively-accurate statistical models to delineate the impact of both undertaken SEU and MBU across layers and per each layer of the selected NN. These models can be used for evaluating the error-resiliency magnitude of NN topology before adopting them in the safety-critical applications.

==> DSN_reviews.tex <==
Overall merit
2. 	Weak reject (Reject, but I won't fight for it)
Novelty
3. 	New contribution
Writing quality
2. 	Needs improvement
Reviewer expertise
3. 	Knowledgeable
Paper summary
The authors propose a simple statistical model to estimate soft error impact on binary neural networks. The approach they leverage is based on fault injection, and then using this input an entropy based model is developed. Results show the correlation between the predicted impact and fault-injection campaign. 
Strengths
Potentially binary neural networks are relatively more prone to impact of soft errors; and the fault injection campaign confirms this. 
Weaknesses
The modeling is problematic, fault injection has methodological issues, the writing needs much improvement. 
Comments for author
I like the overall topic of the paper: soft-errors occurring in binary neural networks has a relatively large impact and is worthy of research, including developing tools such as the modeling tool of the submission to study the impact of these errors.
There are two contributions in the paper: in the first contribution the authors develop a fault injection framework for binarized neural networks. In the second and the main contribution, the authors leverage the results of this empirical fault injection campaign results to construct a simple statistical model so that the impact of the soft errors on a given binarized neural network could predicted without the need for fault injection. I think this is an interesting research area. However, I think the paper needs another revision before it is ready for publication.
First, the organization and writing quality needs to be substantially improved. There are frequent english issues in the text, most specifically in the choice of words: ("transient faults that might lead to the gradual downgrade of the long-running expected NN inference accelerator.", " Based on the results collected in the previous step, we propose an entropy-based model to estimate the impact of the soft errors on the NN architectural.", ...). There are issues with organization as well, for instance the experimental results in section III D lacks information about the application: how many layers, what kind of layers ,... This is given late in the paper in Section V! There are also long and convoluted sentences which hinder the readability of the paper. I propose to have a native english speaker go over the text carefully.
The above organizational and language issues could be addressed in a revised version. However there are other issues that need to be tackled. For example there is a large body of prior related work in Neural Network resiliency that needs to be added, referred analyzed and compared against. I suggest the authors to start from a recent survey paper on NN resilience: "A survey on modeling and improving reliability of DNN algorithms and accelerators" by S. Mittal. Note that this paper includes a survey of modeling reliability (what you are proposing in the paper) as well. Furthermore, you should refer to C. Schorn et al "Automated design of error-resilient and hardware-efficient deep neural networks", B. Salami et al "On the resilience of rtl nn accelerators: Fault characterization and mitigation" and N. Chandramoorthy et al "Resilient Low Voltage Accelerators for High Energy Efficiency".
Also, the result that: " We also noticed that not only the soft errors inconsistently inﬂuence the parameters, but the magnitude of fault-inﬂuence on the accuracy loss is subject to how early the parameters in the consecutive layers are exposed to soft errors." i.e. NN layers are differently impacted by errors: this is well known, please check prior work. 
I also had issues with the methodology: - 100 MBU faults are injected. How likely would those cumulative 100 MBU events be (in which time interval)? The MBU assumes 8 bit corruption - it is too much IMO. - Targeted in-layer fault injection: with what distribution? Each layer size can be different, did you inject the same number of faults for all layers? If so, the fault rate per bit is different. - I dont buy the argument of accumulation of hundreds of soft errors: " However, the accumulated radiation-induced transient faults can potentially impact the individual parameters in NN topology, and if not mitigated immediately, the functionality of a long-running expected NN inference accelerator can gradually downgrade and lead to drastic accuracy loss." How about periodically loading the weight data back? This is similar to cache scrubbing in a way. 
Review #359B
________________________________________
Overall merit
2. 	Weak reject (Reject, but I won't fight for it)
Novelty
3. 	New contribution
Writing quality
2. 	Needs improvement
Reviewer expertise
2. 	Some familiarity
Paper summary
The paper studies precision reduction in neural networks that results from single-event and multi-bit upset scenarios. Such problems can affect the reliability of ML/AI systems and require dedicated characterization. Among others, the authors study the sensitivity of the network accuracy to the layer location, quantization level, and number of faults, partitioning experimental variance across factors. Among the main points raised by the paper is that errors affecting initial layers can propage to consecutive layers and therefore should be considered as more severe. 
Strengths
The paper tackles reliability testing and analysis in neural networks. It produces interesting evidence that the location and types of bit faults can impact in heterogenous manners a neural network accuracy. 
Weaknesses
An initial characterization is developed based on an experimental approach, however the observations throughout do not lead to a coherent methodology to fully characterize and prevent these issues. 
Comments for author
The authors present a well motivated and timely research problem. The points raised at the end of the first page as motivations are interesting and, at least for me, fully agreeable.
A number of interesting experiments, such as those in Fig 3 and 4, illustrate empirically the sensitivity of neural network accuracy to bit perturbations. Section III.B presents the parameters used in these experiments, the authors should however elaborate further on what other parameters may be used and why they have not been considered.
The design of experiments is sensible, however the experimental results indicate that most factors produce negligible interactions. I could not take out much from the tables as they seemed to point at first-order factors as being dominant, so the interactions seemed not very interesting. It is also not clear to me why you haven't tried larger designs (eg fractional factorial designs) to push the scale of the study to more features.
The paper is rather short and does not fully develop the story besides a few numerical tests, for example, how should we shield from these issues? This is my view one of the core limitations of this work.
The background section is really brief, I feel the authors may want to expand it with more details about how these kinds of analyses are carried out in traditional systems.
English is hard to follow in many parts and this reduces the clarity of the message. The authors should avoid repeated use of past tense, proof-read perhaps with the help of some tools. 
Review #359C
________________________________________
Overall merit
1. 	Reject (I will fight to kill the paper)
Novelty
2. 	Incremental improvement
Writing quality
3. 	Adequate
Reviewer expertise
2. 	Some familiarity
Paper summary
The basic contribution of the paper is an entropy-based model that "estimates" the impact of errors on binary neural networks. Their results show that the predicted impact and fault-injection campaign results are similar. 
Strengths
+ the paper attacks an important and challenging problem - with somewhat interesting take. 
Weaknesses
- sub-par writing quality: hurts readability.
- experimental evaluation appears incomplete or very short.
- the proposed model has not been fully developed and its robustness has not been established. 
Comments for author
The paper poses an interesting question: how to estimate the impact of faults without doing a fault injection campaign but rather building a model of it. However, the paper's contribution is limited in many ways. Authors are encouraged to pursue this path of exploration but strengthen the paper in the following aspects:
- please clearly define and use acronyms. The writing is sub-par and it hurts the readability of the paper. 
- the paper is relatively weak on the experimental evaluation side: the impact and benefits are not demonstrated across different models and datasets.
- Section IV : the model itself is hard to understand and it is unclear if it covers all the cases. What is the validation accuracy and its robustness?
- please clearly articulate the novelty of the approach by comparing with other works in this area.


